Exploring regular and turbulent flow states in active nematic channel flow via Exact Coherent Structures and their invariant manifolds

This work is a unified study of stable and unstable steady states of 2D active nematic channel flow using the framework of Exact Coherent Structures (ECS). ECS are stationary, periodic, quasiperiodic, or traveling wave solutions of the governing equations that, together with their invariant manifolds, organize the dynamics of nonlinear continuum systems. We extend our earlier work on ECS in the preturbulent regime by performing a comprehensive study of stable and unstable ECS for a wide range of activity values spanning the preturbulent and turbulent regimes. In the weakly turbulent regime, we compute more than 200 unstable ECS that co-exist at a single set of parameters, and uncover the role of symmetries in organizing the phase space geometry. We provide conclusive numerical evidence that in the preturbulent regime, generic trajectories shadow a series of unstable ECS before settling onto an attractor. Finally, our studies hint at shadowing of quasiperiodic type ECS in the turbulent regime.

==> backup <==
%\begin{table}
%\centering
%\begin{tabular}{p{10mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{10mm}>{\centering\arraybackslash}p{10mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}>{\centering\arraybackslash}p{15mm}}  \hline \hline \addlinespace[2mm]
%$n_x$ & $a/L$ & $\text{Re}(\lambda)$ & & $n_x$ & $a/L$ & $\text{Re}(\lambda)$& & $n_x$ & $a/L$ & $\text{Re}(\lambda)$ \\
%\hline
%\addlinespace[2mm]
%6 & 13.33 & 0.623 & & 10 & 8.0 & 0.372 & & 9 & 8.88 & 0.207\\ 
%7 & 11.42 & 0.603 & & 3 & 26.66 & 0.296 & & 10 & 8.0 & 0.137\\ 
%5 & 16.0 & 0.595 & & 11 & 7.27 & 0.254 & & 12 & 6.66 & 0.12\\ 
%8 & 10.0 & 0.55 & & 7 & 11.42 & 0.249 & & 5 & 16.0 & 0.115\\ 
%4 & 20.0 & 0.497 & & 8 & 10.0 & 0.246 & & 11 & 7.27 & 0.042\\ 
%9 & 8.88 & 0.471 & & 6 & 13.33 & 0.208 & & 2 & 40.0 & -0.021\\ 
%\addlinespace[1mm]
%\hline \hline            
%\end{tabular}
%\caption{Some features of the leading eigenvectors of the dynamics linearized about UNI at Ra = 3.4. The eigenvectors are pure Fourier modes in $x$, of the form $e^{\pm 2\pi n_x/L}$, where $L=80$ is the channel width. $\lambda$ is the Floquet exponent, so positive (negative) $\text{Re}(\lambda)$ means the eigenvector represents an unstable (stable) direction. Also shown is the corresponding length scale $a = L/n_x$.}
%\label{table:UNI_eigenvectors}
%\end{table}

%In between, the phase space can be partitioned into two subdomains: the union of the basins of attraction of the stable ECS, and similarly for any chaotic attractors. 

%If the equilibrium is unstable with respect to a perturbation into one of these subspaces, then applying this perturbation to the initial state with %Using these as initial conditions has the added advantage	
%for some value of activity, there exist attractors with a row of 3-5 identical (or nearly so) vortices. Similarly, any state with a 3-5 fold translation symmetry would be a plausible candidate.  The idea is to use a set of 1D equilibria with degenerate translational symmetry as "entry points" to the various symmet
%The system's attractors tend to inherit certain discrete symmetries from the equations of motion. These symmetries are influenced by the system's %intrinsic length scales. These symmetries are influenced by the system's intrinsic length scales determine which symmetries are dynamically %favorable, and thereby provide a guideline for generalizing to different channel dimensions. 

%Even well-designed search strategies cannot guarantee
%Ideally, the probability of detecting an ECS will be proportional to an objective measure of its dynamical relevance. Our strategy of searching along time-dependent trajectories 
%\begin{itemize}
 %\item State biases of search. Ideally, would want the likelihood of detecting an ECS to be
%	directly proportional to an objective measure of its dynamical relevance
%	In practice, this type of objectivity is difficult to establish.
%	In our case, there are a few biases towards measures besides
%	dynamical relevance.
 %\begin{itemize}
%	\item Bias toward smaller periods. By contrast, Floquet exponents (local divergence near ECS) may matter more for shadowing than Floquet multiplier .. so an ECS doesn't necessarily have to be shadowed for an entire period for its contribution to matter (cite PRL paper that used persistent homology). Newton-Rhapson has to see full ECS (cite PRL paper that used persistent homology)
%\item Especially for larger activity, many ECS were found by symmetry reduction simply because this was easier for Newton-Rhapson
%\item unstable manifolds of 1D equilibria
%\end{itemize}
 %\end{itemize}
 %However, none of these searches should be considered exhaustive. In the presence of chaos, there will generally be an infinite number of ECS with arbitrarily large periods. Moreover, due to the unpredictable convergence behavior of the Newton-Rhapson solver, there is no guarantee that a given (finite) number of searches will uncover all ECS with a given property, such as periods less than some value. On the other hand, by initializing our searches from time-dependent trajectories, we will naturally tend to discover the most dynamically relevant ECS. This fact, combined with other search strategies, 

%However, none of these searches should be considered exhaustive. In the presence of chaos, there will generally be an infinite number of ECS with arbitrarily large periods. Moreover, due to the unpredictable convergence behavior of the Newton-Rhapson solver, there is no guarantee that a given (finite) number of searches will uncover all ECS with a given property, such as periods less than some value. On the other hand, by initializing our searches from time-dependent trajectories, we will naturally tend to discover the most dynamically relevant ECS. This fact, combined with other search strategies, 

%The mosiac image xxx in the Supplement provides a visual overview of many of the flow structures exhibited by unstable ECS, depicting snapshots of all 154 ECS found at $\mathrm{Ra} = 4.5$.

%reiterate typical values for ECS periods, to provide a reference point for the timescales in the figure. Also, explain that figure \ref{fig:R34_phasespace_density_shadowing} only shows a 2D projection and does not evaluate all the shadowing criteria. However, we have checked the rigorous criteria for all the marked ECS, and show a couple of examples.
    
    %Then, highlight the following features:
    %\begin{itemize}
    %\item top left: shadowing of ECS within the "RPOu" family. Briefly note 12-fold traveling wave, and also the fact that some trajectories immediately go to one of the 3-fold RPOs, which is an attractor (hence, not strictly shadowing). However, also note that not all shadowing events in this subplot correspond to ECS in the RPOu category. There appears to be some broader set of ECS, some of which perhaps bifurcated off of the RPOu family at smaller activity (e.g. T5/i-4). Similarly, there appear to be at least two unstable tori that exhibit a lot of shadowing events.
    %\item Middle: Some "RPOu"s still visible; apparently, some shadowing events span many periods.
    %\item New set of ECS becomes important (caution: they may not all be dynamically related in phase space; they just appear clustered in the 2D projection). 
    %\item Three ECS are attractors, so these aren't strictly shadowing events. We instead focus on the unstable ECS. Show/describe example trajectories that hit some of these ECS, perhaps more than one in a single trajectory. 
    %\end{itemize}


%can characterize subh trajectories, which, due to their complicated nonlinear dynamics, are not otherwise susceptible to a reduced-order description.

%This category includes not only turbulent flow at high activity, but also chaotic attractors coexisting with attracting ECS at intermediate activity (figure xxx).

%In this connection, it is useful to think of the set of attractors from section \ref{sec:attractors} as a reduced-order description of long-time, non-chaotic trajectories. In this case, the state of the AN can be described entirely in terms of a handful of equilibria and periodic orbits. Similarly, we hypothesize that a finite set of unstable ECS can provide information on transient and turbulent trajectories, at least approximately and possibly in a statistical sense. 

%Of course, attracting ECS cannot describe other important behavior, such as chaotic flows

%Due to the complex and nonlinear time-dependence of the latter, it is not clear how, or whether, a reduced-order description could be obtained. 


    %\begin{itemize}
    %\item Different definitions of shadowing
    %\begin{enumerate}
    %\item Topological -- Yalniz 2020
    %\item ``Co-evolution" -- Georgia Tech group \cite{krygier2021exact}.
    %\end{enumerate}
    %\item ``Close approach" criterion is insufficient; trajectory must evolve similarly to ECS.
    %\item Current state of the art: experimental detection of shadowing in Taylor-Couette flow using the co-evolution criteria.
    %\end{itemize}
    
    %\subsubsection{Implementation} \label{subsec:shadowing-implementation}
    %\begin{enumerate}
    %\item State specific shadowing criteria as put forward on pages 15--16 of \cite{krygier2021exact}.
    %\item Details of our own implementation
    %\begin{itemize}
    %\item Ignore escape time aspect for present purposes 
    %\item Establish natural distance measure
    %\item Thresholds for the third criterion
    %\end{itemize}
    %\item Code implementation: scipy/cupy minimization
    %\end{enumerate}
    
    %\subsubsection{Shadowing along unstable manifolds}


    %Start with explanation of figure \ref{fig:R34_phasespace_density_shadowing}. As part of this, reiterate typical values for ECS periods, to provide a reference point for the timescales in the figure. Also, explain that figure \ref{fig:R34_phasespace_density_shadowing} only shows a 2D projection and does not evaluate all the shadowing criteria. However, we have checked the rigorous criteria for all the marked ECS, and show a couple of examples.
    
    %Then, highlight the following features:
    %\begin{itemize}
    %\item top left: shadowing of ECS within the "RPOu" family. Briefly note 12-fold traveling wave, and also the fact that some trajectories immediately go to one of the 3-fold RPOs, which is an attractor (hence, not strictly shadowing). However, also note that not all shadowing events in this subplot correspond to ECS in the RPOu category. There appears to be some broader set of ECS, some of which perhaps bifurcated off of the RPOu family at smaller activity (e.g. T5/i-4). Similarly, there appear to be at least two unstable tori that exhibit a lot of shadowing events.
    %\item Middle: Some "RPOu"s still visible; apparently, some shadowing events span many periods.
    %\item New set of ECS becomes important (caution: they may not all be dynamically related in phase space; they just appear clustered in the 2D projection). 
    %\item Three ECS are attractors, so these aren't strictly shadowing events. We instead focus on the unstable ECS. Show/describe example trajectories that hit some of these ECS, perhaps more than one in a single trajectory. 
    %\end{itemize}
    %\subsubsection{Shadowing during sustained turbulence}



%\begin{itemize}
%\item Why don't we see more shadowing in chaotic attractor?
%\begin{enumerate}
%\item Local curvature of chaotic attractor is too high for Newton-Rhapson to converge. (Note that chaotic sets appear already well before the final ECS goes unstable)
%\item Bias toward smaller periods. By contrast, Floquet exponents (local divergence near ECS) may matter more for shadowing than Floquet multiplier .. so an ECS doesn't necessarily have to be shadowed for an entire period for its contribution to matter (cite PRL paper that used persistent homology). Newton-Rhapson has to see full ECS
%\item Possible shadowing of higher order structures such as heteroclinic connections, unstable tori
%\end{enumerate}
%\item In line with the above, future work should try to refine the shadowing criterion to cover cases without visually obvious shadowing .. the end goal should be a nonlinear reduction method that's entirely data driven. Mention that it's challenging but important to develop data reduction methods that are nonlinear and fully time-dependent. Maybe cite the Brunton and Kutz book.
%\end{itemize}

 	%\begin{figure}
    %\includegraphics[width=0.99\textwidth]{figures/shadowing_distances.png}
    %\includegraphics[width=0.49\textwidth]{figures/shadowing2.jpg}
    %\includegraphics[width=0.49\textwidth]{figures/snapshots.jpg}
    %\caption{Example shadowing event. [to-do: write description; check top figure and add labels; add real-space snapshots corresponding to bottom left figure]}
    %    \label{fig:shadowing_example}
    %\end{figure}
